Learning Execution Contexts from System Call Distributions for Intrusion Detection in Embedded Systems

Existing techniques used for intrusion detection do not fully utilize the intrinsic properties of embedded systems. In this paper, we propose a lightweight method for detecting anomalous executions using a distribution of system call frequencies. We use a cluster analysis to learn the legitimate execution contexts of embedded applications and then monitor them at run-time to capture abnormal executions. We also present an architectural framework with minor processor modifications to aid in this process. Our prototype shows that the proposed method can effectively detect anomalous executions without relying on sophisticated analyses or affecting the critical execution paths.

==> Motivation.tex <==
%\section{Motivation}\label{sec::motivation}

==> syscall_related.tex <==
\section{Related Work}
\label{sec::related}


Forrest \textit{et al.}~\cite{Forrest:1996} build a database of look-ahead pairs of system calls; for each system call type, what is the next $i^{th}$ system call for $i=1,2,$ up to $N$. Then, given a longer sequence of length $L>N$, the percentage of mismatches is used as the metric to determine abnormality. Hofmeyr \textit{et al.}~\cite{Hofmeyr:1998} extends the method by profiling unique sequences of \emph{fixed} length $N$, called \emph{N-gram}, to reduce the database size. The legitimacy test for a given sequence of length $N$ is carried out by calculating the smallest Hamming distance between it and the all sequences in the database. %This fundamental model evolved in various aspects in follow-up work. For example, 
The N-gram model requires a prior assumption on suitable $N$ because it affects the accuracy as well as the database size. Marceau \cite{Marceau:2000} proposes a finite state machine (FSM) based prediction model to relax these requirements and Eskin \textit{et al.}~\cite{Eskin01modelingsystem} further improves by employing a \emph{wild-card} for compact sequence representation. Other prediction models such as Hidden Markov model (HMM) \cite{Warrender99detectingintrusion} and Markov chains \cite{Jha:2001} have also been explored. A similar approach to our work is \cite{Burguera:2011}, in which the system call counts of Android applications (traced by a software tool called \emph{strace}) are used to find malicious apps. Using a crowdsourcing, the approach collects the system call counts of a particular application from multiple users and applies $k$-means (with Euclidean distance metric) to divide them into \emph{two} clusters. A smaller cluster is considered to be malicious based on the assumption that benign apps are the majority. 


%Forrest \textit{et al.}~\cite{Forrest:1996} build a database of look-ahead pairs of system calls; for each system call type, what is the next $i^{th}$ system call for $i=1,2,$ up to $N$. Then, given a longer sequence of length $L>N$, the percentage of mismatches is used as the metric to determine abnormality. Hofmeyr \textit{et al.}~\cite{Hofmeyr:1998} extends the method by profiling unique sequences of \emph{fixed} length $N$, called \emph{N-gram}, to reduce the database size. The legitimacy test for a given sequence of length $N$ is carried out by calculating the smallest Hamming distance between it and the all sequences in the database. This fundamental model evolved in various aspects in follow-up work. For example, the N-gram model requires a prior assumption on suitable $N$ because it affects the accuracy as well as the database size. Marceau \cite{Marceau:2000} proposes a finite state machine (FSM) based prediction model to relax these requirements; it can predict the next system call given a sequence consisting of the last $N$ system calls, where $N$ varies with the sequence. Eskin \textit{et al.}~\cite{Eskin01modelingsystem} further improves by modeling legitimate sequences as a mixture of prediction trees, in which a \emph{wild-card} is employed to represent sequences in a compact and flexible way. Other prediction models such as Hidden Markov model (HMM) \cite{Warrender99detectingintrusion} and Markov chains \cite{Jha:2001} have also been explored. A similar approach to our work is \cite{Burguera:2011}, in which the system call counts of Android applications (traced by a software tool called \emph{strace}) are used to find malicious apps. Using a crowdsourcing, the approach collects the system call counts of a particular application from multiple users and applies $k$-means (with Euclidean distance metric) to divide them into \emph{two} clusters. A smaller cluster is considered to be malicious based on the assumption that benign apps are the majority. 


There has also been work on system call arguments monitoring. Mutz \textit{et al.}~\cite{Mutz:2006} introduce several techniques to test anomalies in argument lengths, character distribution, argument grammar, \textit{etc.} Maggi \textit{et al.} \cite{Maggi:2010} use a clustering algorithm to group system call invocations that have similar arguments. 

%As previously mentioned, the usual way of system call instrumentation relies on an audit module in the OS layer. 
Hardware-based system call monitoring mechanism can improve the overall security of the 
system by cutting off a potential vulnerability -- the software audit module. Pfoh \etal \cite{Pfoh:2011} proposed Nitro, a hardware-based system call tracing system where system calls made inside virtual machines in manner similar to ours (Section~\ref{sec::sctm}). We note that our detection method (Section~\ref{sec::analysis}) is orthogonal to how system calls are traced. Hence we can 
implement it on systems like Nitro. %Other types of instrumentation include static analysis of program source code \cite{Wagner:2001} and user-level processes for system call interposition \cite{Jain:1999}.


The SecureCore architecture~\cite{yoonsecurecore2013} takes advantage of the \emph{redundancy} of 
a multicore processor; a \emph{secure core} is used to monitor the run-time execution behavior of target applications running on a \emph{monitored core}. The original architecture is designed to watch applications \emph{timing} behavior. There also exists some work in which a multicore processor (or a coprocessor) is employed as 
a security measure, such as \cite{Deng:2010,embeddedsecurity:s3a2012, Lo:2014}.%, for instruction-grain monitoring. 
%\cite{Chen:2008, Kannan:2009, Deng:2010,embeddedsecurity:s3a2012}, for instruction-grain monitoring. 

%,

%------------------
%
%A Comparison with Gaussian Kernel Density Estimator
%
%-----------------
%
%% Jaesik: you can put this either in introduction or related work.
%
%Our method includes improvements over the recent non-parametric method \cite{Securecore2012} in two key aspects. The (Gaussian) kernel density estimator is modeled on one-dimension (time of executions of a computational unit). This method enables modeling system call distributions which are collected from multi-dimensions features.  Another main drawbacks of non-parametric methods are that the number of parameters increases as training data increase. Data reduction methods such as collapsed Gaussian mixture \cite{Goldberger2005} handle the issues by the bottom-up clustering from individual Gaussians to a small numbers of clusters. Here, the global k-means clustering algorithm also reduces the number of parameters by the top-down approach.
%
%-----------------
%
%
